Blowing bubbles on the torus

We consider the regularized trace of the inverse of the Laplacian on a skinny torus. With its flat metric, a skinny torus has large trace, but we show that there are conformally equivalent metrics making the trace close to that of a sphere of the same area. This behavior is in sharp contrast to that of the log-determinant, a well-known spectral invariant which is extremized at the flat metric on any torus. Our examples are bubbled tori, where you take a sphere, discard polar regions, and glue top to bottom. In a addendum, we belatedly notice that our bubbled tori have trace less than the sphere, and outline how to exploit this to get Okikiolu's result that by means of a conformal factor depending only on longitude, any torus can be made to have trace less than the sphere.

==> bubble_dot_bib <==
@book {Aldousfill,
	AUTHOR={Aldous, David and Fill, Jim},
	TITLE={Reversible Markov Chains and Random Walks on Graphs},
	NOTE={\url{http://www.stat.berkeley.edu/users/aldous/RWG/book.html}},
	YEAR={2002},
}

@book {Aubin,
    AUTHOR = {Aubin, Thierry},
     TITLE = {Some nonlinear problems in {R}iemannian geometry},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {1998},
     PAGES = {xviii+395},
      ISBN = {3-540-60752-8},
}

@article {Chiu,
    AUTHOR = {Chiu, Patrick},
     TITLE = {Height of flat tori},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {125},
      YEAR = {1997},
    NUMBER = {3},
     PAGES = {723--730},
      ISSN = {0002-9939},
     CODEN = {PAMYAR},
   MRCLASS = {58G26 (11E45)},
  MRNUMBER = {MR1396970 (97g:58173)},
MRREVIEWER = {Jack Quine},
}

@article {Diaconisstroock,
    AUTHOR = {Diaconis, Persi and Stroock, Daniel},
     TITLE = {Geometric bounds for eigenvalues of {M}arkov chains},
   JOURNAL = {Ann. Appl. Probab.},
  FJOURNAL = {The Annals of Applied Probability},
    VOLUME = {1},
      YEAR = {1991},
    NUMBER = {1},
     PAGES = {36--61},
      ISSN = {1050-5164},
   MRCLASS = {60J10},
  MRNUMBER = {MR1097463 (92h:60103)},
MRREVIEWER = {Gregory F. Lawler},
}

 @article {Morpurgo,
    AUTHOR = {Morpurgo, C.},
     TITLE = {The logarithmic {H}ardy-{L}ittlewood-{S}obolev inequality and
              extremals of zeta functions on ${S}\sp n$},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {6},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {146--171},
      ISSN = {1016-443X},
 }
 
 @article {Morpurgo_Duke,
    AUTHOR = {Morpurgo, Carlo},
     TITLE = {Sharp inequalities for functional integrals and traces of
              conformally invariant operators},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {114},
      YEAR = {2002},
    NUMBER = {3},
     PAGES = {477--553},
      ISSN = {0012-7094},
}



@article {Ops,
    AUTHOR = {Osgood, B. and Phillips, R. and Sarnak, P.},
     TITLE = {Extremals of determinants of {L}aplacians},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {80},
      YEAR = {1988},
    NUMBER = {1},
     PAGES = {148--211},
      ISSN = {0022-1236},
 }



@article {Okikiolu,
    AUTHOR = {Okikiolu, K.},
     TITLE = {Critical metrics for the determinant of the {L}aplacian in odd
              dimensions},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {153},
      YEAR = {2001},
    NUMBER = {2},
     PAGES = {471--531},
}

@article {Okikiolububble,
    AUTHOR = {Okikiolu, K.},
     TITLE = {A negative mass theorem for the 2-torus},
       eprint = {arXiv:0711.3489v1 [math.SP]},
       YEAR={2007},
}

@article {Okikiolutrace,
    AUTHOR = {Okikiolu, K.},
     TITLE = {Extremals for logarithmic {H}ardy-{L}ittlewood-{S}obolev inequalities on compact manifolds},
       eprint = {arXiv:math/0603717v1 [math.SP]},
       YEAR={2006},
}

@article {Richardson,
    AUTHOR = {Richardson, Ken},
     TITLE = {Critical points of the determinant of the {L}aplace operator},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {122},
      YEAR = {1994},
    NUMBER = {1},
     PAGES = {52--83},
      ISSN = {0022-1236},
     CODEN = {JFUAAW},
   MRCLASS = {58G26 (58E11)},
  MRNUMBER = {95j:58176},
MRREVIEWER = {Paul C. Yang},
}


@book {Taylor1,
    AUTHOR = {Taylor, Michael E.},
     TITLE = {Partial differential equations. {I}},
    SERIES = {Applied Mathematical Sciences},
    VOLUME = {115},
      NOTE = {Basic theory},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {New York},
      YEAR = {1996},
     PAGES = {xxiv+563},
      ISBN = {0-387-94653-5},
   MRCLASS = {35-01 (46N20 47N20 58Gxx)},
  MRNUMBER = {98b:35002b},
MRREVIEWER = {Luigi Rodino},
}


 @article {steiner_duke,
    AUTHOR = {Steiner, Jean},
     TITLE = {A geometrical mass and its extremal properties for metrics on {$S\sp 2$}},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {129},
      YEAR = {2005},
    NUMBER = {1},
     PAGES = {63--86},
}



@article{hideandseek,
AUTHOR={Doyle, Peter and Steiner, Jean},
TITLE={Spectral invariants and playing hide-and-seek on surfaces},
YEAR = {2005},
%eprint={arXiv:XXXX.YYYYv1 [math.SP]},
}


@article {Leveneloizou,
    AUTHOR = {Levene, Mark and Loizou, George},
     TITLE = {Kemeny's constant and the random surfer},
   JOURNAL = {Amer. Math. Monthly},
  FJOURNAL = {The American Mathematical Monthly},
    VOLUME = {109},
      YEAR = {2002},
    NUMBER = {8},
     PAGES = {741--745},
      ISSN = {0002-9890},
     CODEN = {AMMYAE},
   MRCLASS = {60J10 (60E15)},
  MRNUMBER = {MR1927624 (2003e:60162)},
MRREVIEWER = {Vivek S. Borkar},
}

@book {Kemenysnell,
    AUTHOR = {Kemeny, John G. and Snell, J. Laurie},
     TITLE = {Finite {M}arkov chains},
    SERIES = {The University Series in Undergraduate Mathematics},
 PUBLISHER = {D. Van Nostrand Co., Inc., Princeton, N.J.-Toronto-London-New
              York},
      YEAR = {1960},
     PAGES = {viii+210},
   MRCLASS = {60.00},
  MRNUMBER = {MR0115196 (22 \#5998)},
MRREVIEWER = {K. L. Chung},
}


@book {RWEN,
    AUTHOR = {Doyle, Peter and Snell, J. Laurie},
     TITLE = {Random walks and electric networks},
    SERIES = {Carus Mathematical Monographs},
    VOLUME = {22},
 PUBLISHER = {Mathematical Association of America},
   ADDRESS = {Washington, DC},
      YEAR = {1984},
     PAGES = {xiv+159},
      ISBN = {0-88385-024-9},
   MRCLASS = {94C05 (60J15 94C15)},
  MRNUMBER = {MR920811 (89a:94023)},
MRREVIEWER = {H. Kesten},
}

@article {Meyer,
    AUTHOR = {Meyer, Jr., Carl D.},
     TITLE = {The role of the group generalized inverse in the theory of
              finite {M}arkov chains},
   JOURNAL = {SIAM Rev.},
  FJOURNAL = {SIAM Review},
    VOLUME = {17},
      YEAR = {1975},
     PAGES = {443--464},
      ISSN = {1095-7200},
   MRCLASS = {60J10},
  MRNUMBER = {MR0383538 (52 \#4419)},
MRREVIEWER = {E. Seneta},
}

@book {Hsu,
    AUTHOR = {Hsu, Elton P.},
     TITLE = {Stochastic analysis on manifolds},
    SERIES = {Graduate Studies in Mathematics},
    VOLUME = {38},
 PUBLISHER = {American Mathematical Society},
   ADDRESS = {Providence, RI},
      YEAR = {2002},
     PAGES = {xiv+281},
      ISBN = {0-8218-0802-8},
   MRCLASS = {58J65 (60-02 60G48 60H05 60H10 60J60 60J65)},
  MRNUMBER = {MR1882015 (2003c:58026)},
MRREVIEWER = {Yu. E. Gliklikh},
}

@unpublished{Doyle_Kemeny,
AUTHOR={Doyle, Peter},
TITLE={Kemeny's Constant},
NOTE = {\url{ http://math.dartmouth.edu/~doyle/docs/kc/kc.pdf}}, 
YEAR = {2003},
}


@inproceedings{Lovaszwinkler,
 author = {Lovasz, Laslo and Peter Winkler},
 title = {Efficient stopping rules for Markov chains},
 booktitle = {STOC '95: Proceedings of the twenty-seventh annual ACM
symposium on Theory of computing},
 year = {1995},
 isbn = {0-89791-718-9},
 pages = {76--82},
 location = {Las Vegas, Nevada, United States},
 doi = {http://doi.acm.org/10.1145/225058.225086},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }	

@book {Grinsteadsnell,
    AUTHOR = {Grinstead, Charles M. and Snell, J. Laurie},
     TITLE = {Introduction to Probability: Second Revised Edition},
 PUBLISHER = {American Mathematical Society},
   ADDRESS = {Providence, Rhode Island, United States},
      YEAR = {1997},
     PAGES = {xi+510},
      ISBN = {0-8218-0749-8},
}

@article {Carlenloss,
    AUTHOR = {Carlen, E. and Loss, M.},
     TITLE = {Competing symmetries, the logarithmic {H}{L}{S} inequality and
              {O}nofri's inequality on ${S}\sp n$},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {2},
      YEAR = {1992},
    NUMBER = {1},
     PAGES = {90--104},
      ISSN = {1016-443X},
 }

@article {Beckner,
    AUTHOR = {Beckner, William},
     TITLE = {Sharp {S}obolev inequalities on the sphere and the
              {M}oser-{T}rudinger inequality},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {138},
      YEAR = {1993},
    NUMBER = {1},
     PAGES = {213--242},
      ISSN = {0003-486X},
 }

@article {Raysinger,
    AUTHOR = {Ray, D. B. and Singer, I. M.},
     TITLE = {{$R$}-torsion and the {L}aplacian on {R}iemannian manifolds},
   JOURNAL = {Advances in Math.},
    VOLUME = {7},
      YEAR = {1971},
     PAGES = {145--210},
   MRCLASS = {58F20 (53C20)},
  MRNUMBER = {45 \#4447},
MRREVIEWER = {J. W. Robbin},
}

@article {Polyakov1,
    AUTHOR = {Polyakov, A. M.},
     TITLE = {Quantum geometry of fermionic strings},
   JOURNAL = {Phys. Lett. B},
  FJOURNAL = {Physics Letters. B},
    VOLUME = {103},
      YEAR = {1981},
    NUMBER = {3},
     PAGES = {211--213},
      ISSN = {0031-9163},
     CODEN = {PYLBA},
   MRCLASS = {81E99 (58D30 81G20 82A68)},
  MRNUMBER = {84h:81093b},
}
@article {Polyakov2,
    AUTHOR = {Polyakov, A. M.},
     TITLE = {Quantum geometry of bosonic strings},
   JOURNAL = {Phys. Lett. B},
  FJOURNAL = {Physics Letters. B},
    VOLUME = {103},
      YEAR = {1981},
    NUMBER = {3},
     PAGES = {207--210},
      ISSN = {0031-9163},
     CODEN = {PYLBA},
   MRCLASS = {81E99 (58D30 81G05 82A68)},
  MRNUMBER = {84h:81093a},
}


